Vector-based Efficient Data Hiding in Encrypted Images via Multi-MSB Replacement

As an essential technique for data privacy protection, reversible data hiding in encrypted images (RDHEI) methods have drawn intensive research interest in recent years. In response to the increasing demand for protecting data privacy, novel methods that perform RDHEI are continually being developed. We propose two effective multi-MSB (most significant bit) replacement-based approaches that yield comparably high data embedding capacity, improve overall processing speed, and enhance reconstructed images' quality. Our first method, Efficient Multi-MSB Replacement-RDHEI (EMR-RDHEI), obtains higher data embedding rates (DERs, also known as payloads) and better visual quality in reconstructed images when compared with many other state-of-the-art methods. Our second method, Lossless Multi-MSB Replacement-RDHEI (LMR-RDHEI), can losslessly recover original images after an information embedding process is performed. To verify the accuracy of our methods, we compared them with other recent RDHEI techniques and performed extensive experiments using the widely accepted BOWS-2 dataset. Our experimental results showed that the DER of our EMR-RDHEI method ranged from 1.2087 bit per pixel (bpp) to 6.2682 bpp with an average of 3.2457 bpp. For the LMR-RDHEI method, the average DER was 2.5325 bpp, with a range between 0.2129 bpp and 6.0168 bpp. Our results demonstrate that these methods outperform many other state-of-the-art RDHEI algorithms. Additionally, the multi-MSB replacement-based approach provides a clean design and efficient vectorized implementation.

==> figures/AMP.tex <==
\begin{figure}[H]
\centering

    \scalebox{.85}{\input{graphs/AMP}}
    
    \vspace{0.2cm}  
    
    \caption{Adaptive MSB prediction structure}
    \label{fig:amp}
    
    \vspace{-0.2cm}
    
\end{figure}

==> figures/GAP.tex <==
\begin{figure}[H]
\centering

    \scalebox{.7}{\input{graphs/GAP}}
    
    \vspace{0.2cm}  
    
    \caption{Neighboring pixels used in the prediction algorithm}
    \label{fig:GAP}
    
    \vspace{-0.2cm}
    
\end{figure}

==> figures/MED_predictor.tex <==
\begin{figure}[H]
\centering

    \scalebox{.7}{\input{graphs/MED_predictor.tex}}
    
    \vspace{0.2cm}  
    
    \caption{The context of the MED predictor}
    \label{fig:MED_predictor}
    
    \vspace{-0.2cm}
    
\end{figure}

==> figures/Original_image.tex <==
\begin{figure}[H]
\centering

    \scalebox{.7}{\input{graphs/Original_image}}
    
    % \vspace{0.2cm}  
    
    \caption{Original image}
    \label{fig: original_image}
    
    \vspace{-0.2cm}
    
\end{figure} 

==> figures/PEE.tex <==
\begin{figure}[H]
\centering

    \scalebox{.7}{\input{graphs/PEE}}
    
    \vspace{0.2cm}  
    
    \caption{Prediction error estimation (PEE) structure}
    
    \vspace{-0.2cm}
    
\end{figure}

==> imports.tex <==
% IEEE notice
\makeatletter
\def\ps@IEEEtitlepagestyle{%
  \def\@oddfoot{\mycopyrightnotice}%
  \def\@oddhead{\hbox{}\@IEEEheaderstyle\leftmark\hfil\thepage}\relax
  \def\@evenhead{\@IEEEheaderstyle\thepage\hfil\leftmark\hbox{}}\relax
  \def\@evenfoot{}%
}
\def\mycopyrightnotice{%
  \begin{minipage}{\textwidth}
  \centering \scriptsize
  Copyright © 2022 IEEE. Personal use of this material is permitted. However, permission to use this material for any other purposes must be obtained from the IEEE by sending an email to pubs-permissions@ieee.org. DOI: 10.1109/TCSVT.2022.3183391
  \end{minipage}
}

% Imports
\usepackage[dvipsnames]{xcolor}

% For enumerate
\usepackage{enumitem}
% Paper-specific information
\newcommand{\emrMinDER}{1.2087}
\newcommand{\emrAverageDER}{3.2457}
\newcommand{\emrMaxDER}{6.2682}

\newcommand{\lmrMinDER}{0.2129}
\newcommand{\lmrAverageDER}{2.5325}
\newcommand{\lmrMaxDER}{6.0168}

\newcommand{\emrMinPSNR}{51.1108}
\newcommand{\emrAveragePSNR}{51.1409}
\newcommand{\emrMaxPSNR}{51.1723}

\newcommand{\emrMinSSIM}{0.9746}
\newcommand{\emrAverageSSIM}{0.9958}
\newcommand{\emrMaxSSIM}{0.9997}

% For logic
\usepackage{ifthen}

% For Citing and inline stuff
% \usepackage{cite}
\usepackage[numbers]{natbib} % http://merkel.texture.rocks/Latex/natbib.php
\bibliographystyle{plainnat}
\usepackage{url}
\setlength{\bibsep}{2pt}

% For Tables
\usepackage{multirow}
\usepackage{floatrow}
\floatsetup[table]{capposition=bottom}
% \usepackage{booktabs}
% \usepackage{stackengine}
\usepackage{tabularx, makecell}
\usepackage{makecell}
\usepackage{diagbox}
\usepackage{tabularx}
\usepackage{booktabs}

% Created a thicker hline
\makeatletter
\def\thickhline{%
  \noalign{\ifnum0=`}\fi\hrule \@height \thickarrayrulewidth \futurelet
   \reserved@a\@xthickhline}
\def\@xthickhline{\ifx\reserved@a\thickhline
               \vskip\doublerulesep
               \vskip-\thickarrayrulewidth
             \fi
      \ifnum0=`{\fi}}
\makeatother

\newlength{\thickarrayrulewidth}
\setlength{\thickarrayrulewidth}{2\arrayrulewidth}

% For Figures
\usepackage{tikz}
\usepackage{adjustbox}
% \usepackage{subcaption} 
\usepackage{graphicx}
\usepackage{etoolbox}
\usepackage{datatool}
\usepackage{bchart}
\usepackage{subfig}
\usetikzlibrary{shapes.geometric}

% For general math
\usepackage{amsmath}
\usepackage{verbatim}
\usepackage{commath}
\usepackage{bm}
\usepackage{cases}
\usepackage{mathtools}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter{\nint}\lfloor\rceil
\DeclareMathOperator*{\argmax}{argmax}

% For algorithm figures
\usepackage[ruled, vlined]{algorithm2e}

% For symbols
\usepackage{amssymb}

% Tikz Management
\usetikzlibrary{arrows.meta, chains, matrix, patterns}

% Created a custom size font between scriptsize and tiny
\makeatletter
\newcommand\notsotiny{\@setfontsize\notsotiny{6}{7}}
\makeatother

\hyphenation{optical networks semiconductor}

\usepackage{pgfplots}
\pgfplotsset{compat=1.16}

% Source: https://www.reddit.com/r/LaTeX/comments/f59tpr/color_change_natbib_citations/
\usepackage{hyperref}
\usepackage{cleveref}
\hypersetup{colorlinks, citecolor=green, linkcolor=Red, urlcolor=Blue}

==> tables/Features.tex <==
\renewcommand{\arraystretch}{1.5}

\begin{table}[ht]

    % Table formatting
    \centering
    \scriptsize
    
    \begin{center}
        \begin{tabular}{ |c|c|c|c|c|c| }
            \hline
            \multicolumn{2}{|c|}{\diagbox{Methods}{Features}} 
                                                    & separable  & \makecell{error-free \\ data \\ extraction} & \makecell{error-free \\ image \\ recovery} & RRBE \\
            \hline
            \multicolumn{2}{|c|}{\citet{XZhang2012}}     
                                                    & Yes & Yes & No & No   \\
            \hline
            \multicolumn{2}{|c|}{\citet{KMa2013}}    
                                                    & Yes & Yes & Yes & Yes         \\
            \hline
            \multicolumn{2}{|c|}{\citet{XCao2016}}     
                                                    & Yes & Yes & Yes & Yes    \\
            \hline
            \multicolumn{2}{|c|}{\citet{Hong2012}}    
                                                    & No & No & No & No         \\
            \hline
            \multicolumn{2}{|c|}{\citet{YPuyang2018}}    
                                                    & Yes & Yes & Yes & Yes        \\
            \hline
            \multicolumn{2}{|c|}{\citet{ZQian2016}}    
                                                    & Yes & Yes & Yes & No         \\
            \hline
            \multirow{2}{*}{\makecell{Wu \\ et al.\citep{XWu2014}}} 
                                &   Joint       & No & No & No & No    \\
                                \cline{2-6}
                                &   Separable       & Yes & Yes & No & No  \\
            \hline
            \multirow{2}{*}{\makecell{Zhang \\ et al.\citep{XZhang2016}}} 
                                &   Lossless       & Yes & Yes & Yes & No    \\
                                \cline{2-6}
                                &   Reversible       & Yes & Yes & Yes & Yes   \\
            \hline
            \multirow{2}{*}{\makecell{Puteaux \\ et al. \citep{Puteaux2018}}} 
                                &   CPE-HCRDH       & Yes & Yes & No & Yes    \\
                                \cline{2-6}
                                &   EPE-HCRDH       & Yes & Yes  & Yes  & Yes   \\
            \hline
            \multirow{2}{*}{\makecell{Asad \\ et al.\citep{Asad2020}}} 
                                &   with LM & Yes & Yes & Yes & Yes    \\
                                \cline{2-6}
                                &   without LM & Yes & Yes & No & Yes   \\
            \hline
            \multicolumn{2}{|c|}{\textbf{EMR-RDHEI}}    & \textbf{Yes}    & \textbf{Yes}    & \textbf{No}    & \textbf{Yes}   \\
            \hline
            \multicolumn{2}{|c|}{\textbf{LMR-RDHEI}}        & \textbf{Yes}    & \textbf{Yes}    & \textbf{Yes}  & \textbf{Yes} \\
            \hline
            
        \end{tabular}
    \end{center}
    
    % Fixing spacing
    \vspace{-0.20cm}
    
    % Table's information
    \caption{A comparison of features with published methods}
    \label{Tab:Features}

\end{table}

\renewcommand{\arraystretch}{1}



==> test.tex <==
\subsection{Optimal Location map }

In order to achieve the maximum data hiding rate for an image and generate its optimal location map, we need to calculate the highest possible embedding rate. For our first method EMR-RDHEI, $b$ ranges from 2 to 7 since we need to embed the location map into the least significant bit (LSB) plane. For the second method LMR-RDHEI, we will use the JBIG-KIT compression library \citep{JBIG-KIT} to compress the MSB plane and location map together, and store it back to the MSB plane. Therefore, $b$ could range from 2 to 8. 

Given any gray-level image of size $M \times N$, to generate a location map, we should consider the correlation between the neighboring pixels. Let's set $b = 2$ first, in an example image Lena of size $512 \times 512$, 



In order to find the most optimal $b$, we use the equation as the following:
\begin{align}
    b &= [\arg \max_{k} \frac{1}{M \times N} \sum_{i = 0}^{M}\sum_{j = 0}^{N}\mathbb{I}(\mathcal{L}(i,j,k) = 0) \times b] + 2, b = k+2\\
    &= \arg \max_{k} \frac{b}{M \times N} \sum_{i = 0}^{M}\sum_{j = 0}^{N}\mathbb{I}(\mathcal{L}(i,j,k) = 0) \quad b \in [2, 7], b \in \mathbb{Z}
\end{align} Where $\mathbb{I}$ is the indicator and $\mathcal{L}$ is the generated location map.

Furthermore, we proposed another possible way to find value $b$ faster using machine learning model - Support Vector Classifier (SVC), which will be discussed in the Section IV-.

% \subsubsection{Generate the location map $\mathbf{L}$}

